Pre-trained Summarization Distillation

Recent state-of-the-art approaches to summarization utilize large pre-trained Transformer models. Distilling these models to smaller student models has become critically important for practical use; however there are many different distillation methods proposed by the NLP literature. Recent work on distilling BERT for classification and regression tasks shows strong performance using direct knowledge distillation. Alternatively, machine translation practitioners distill using pseudo-labeling, where a small model is trained on the translations of a larger model. A third, simpler approach is to 'shrink and fine-tune' (SFT), which avoids any explicit distillation by copying parameters to a smaller student model and then fine-tuning. We compare these three approaches for distillation of Pegasus and BART, the current and former state of the art, pre-trained summarization models, and find that SFT outperforms knowledge distillation and pseudo-labeling on the CNN/DailyMail dataset, but under-performs pseudo-labeling on the more abstractive XSUM dataset. PyTorch Code and checkpoints of different sizes are available through Hugging Face transformers here http://tiny.cc/4iy0tz.

==> cut_beam.tex <==
% \subsection{Beam Analysis}
% Many MT Distillation papers, \footcite{Kim_2016} have found that, after training students on pseudo-labels that were generated with beam search, students models can reproduce beam search outputs with 1 beam. We cannot replicate this finding on our students and teachers. Table \ref{FIXME} shows that in the three settings we tested the students benefit from increasing the number of beams used in beam search to the level used\footnote{Or rather, suggested by the authors of the paper associated with the teacher. 6 for BART and 8 for Pegasus.} by the teacher. This is true for students trained on pseudo-labels and students trained on the original data.
